Interfacing Foundation Models' Embeddings

Foundation models possess strong capabilities in reasoning and memorizing across modalities. To further unleash the power of foundation models, we present FIND, a generalized interface for aligning foundation models' embeddings with unified image and dataset-level understanding spanning modality and granularity. As shown in the teaser figure, a lightweight transformer interface without tuning any foundation model weights is enough for segmentation, grounding, and retrieval in an interleaved manner. The proposed interface has the following favorable attributes: (1) Generalizable. It applies to various tasks spanning retrieval, segmentation, etc., under the same architecture and weights. (2) Interleavable. With the benefit of multi-task multi-modal training, the proposed interface creates an interleaved shared embedding space. (3) Extendable. The proposed interface is adaptive to new tasks, and new models. In light of the interleaved embedding space, we introduce FIND-Bench, which introduces new training and evaluation annotations to the COCO dataset for interleaved segmentation and retrieval. We are the first work aligning foundations models' embeddings for interleave understanding. Meanwhile, our approach achieves state-of-the-art performance on FIND-Bench and competitive performance on standard retrieval and segmentation settings.

==> algos/data_engine.tex <==
\begin{figure}[t]
    \begin{algorithm}[H]
      \scriptsize      
  \Function{data\_engine(llava\_cap,coco\_cap,coco\_pano,lvis\_inst)}{
     \var{Content = \textcolor{gray}{```}generate image captions with grounded entities and attributes with following: }\\
     \var{\textcolor{blue}{pseudo image description}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;  \; \;\; \; \; \; \; \; \; \;  \; \;  \; \;}\\
     \var{\textcolor{blue}{ground truth image captions}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;  \; \; }\\
     \var{ground truth bounding boxes (x0,y0,w,h): (x0,y0) is the coordinate of the top-left corner, (w,h) is box size), \\
     \textcolor{blue}{category\_info, and entity\_id}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;}\\
     \var{\textcolor{blue}{entity\_proposal}: <\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \; \; \; \;  \; \; \;  \; \;}\\
     \var{an example output format would be: "(entity\_id)<A woman> sitting next to (entity\_id)<a handsome man>, with their hands holding together under (entity\_id)<the blue sky>.", where \textbf{(entity\_id)~and~<xxx>~are associated with the ground truth bounding boxes. entity\_id is the real id number in the ground truth bounding boxes.} generated caption constraints:~1.~xxx; 2.~xxx; \textcolor{gray}{'''}.\\ \textcolor{red}{format}(llava\_cap, coco\_cap, coco\_pano, lvis\_inst))
     };
     
     \var{output = GPT4(content)}
     }
      \caption{Pseudo code for Data Engine.}
      \label{alg:shared_initialization}
  \end{algorithm}
\end{figure}

==> figures/benchmark.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/bench.pdf}
    \vspace{-20pt}
    \caption{Example ground truth for FIND-Bench. (a) Grounded captions for COCO-Entity training set. (b) Grounded captions together with interleaved visual references for COCO-Entity validation set. (c) Grounded captions for COCO-Paragraph validation set. (The interleaved visual references are omitted due to space limit.)}
    \label{fig:bench}
    \vspace{-15pt}
\end{figure*}

==> sec/3_benchmark.tex <==
% \section{Benchmark}
\vspace{-8pt}
\section{\textit{FIND} Bench}
\vspace{-5pt}

\input{figures/benchmark}

In order to evaluate the capability of interleaved visual understanding, we propose a new benchmark called \textbf{FIND-Bench}. This includes a fully annotated dataset for both training and evaluation, featuring pairs of images and interleaved entity-based query, as shown in Fig.~\ref{fig:bench}. FIND-Bench supports two new tasks, interleaved image retrieval and interleaved grounded segmentation, which we introduce in detail below.

\vspace{-5pt}
\subsection{Task Definition}

\textbf{Interleaved Image Retrieval}
Let $I$ and $T$ denote image and text, respectively. 
We define a search query as a sequence $Q = \{q_1, q_2, \ldots, q_n\}$, where $q_k$ can be either an instance of $I_i$ or $T_j$. An example could be ``A person with a red shirt is playing with [IMAGE] on the grassland.'', where [IMAGE] is an image. The search space, represented as $S = \{I_1, I_2, \ldots, I_m\}$, is an image dataset.

\vspace{1mm}\noindent
\textbf{Interleaved Grounded Segmentation}
Similar to interleaved image retrieval, we again define $I$ as images, $S, T$ as texts, where $I, S$ represents entities (e.g. image reference, ``a person''), and $T$ represents text connections. The search query is formulated as a sequence $Q = \{q_1, q_2, \ldots, q_n\}$, $ q_i \in \{I, S, T\}$. And the search space is all the segments for an image $\{o_1, o_2, \ldots\,o_n\}$. The objective is to find the corresponding $o_i$ in the image for each instance of $I, S$ in the query $Q$.

\vspace{-8pt}
\subsection{Dataset}
\textbf{Data Engine} We create this new dataset on COCO images with ground truth labels, including captions and panoptic segmentation annotations. 
In addition, we leverage LLaVA~\cite{liu2023visual} to generate detailed captions as instance-level pseudo-ground truth, and GPT4 as the augmentation engine.
We show the pseudo-code of the data engine in Algo.~\textcolor{red}{1}, where GPT4 takes in all provided text information to generate entity-associated captions. Finally,  we use SEEM to find the most visual-like cross-image instance for the labeled entity in each image. The pseudo-ground truths are verified by humans for quality control.

\noindent
\textbf{Statistics} As shown in the table below, our proposed dataset contains 118k training images, 5k validation images, together with 300k training captions, and 1000k training entities. Notably, each entity is associated with a bounding box, mask, phrase, or visual reference to support both text and interleaved grounding.


\input{algos/data_engine}
\input{tables/statistics}
\input{tables/table1}

==> tables/ablation2.tex <==
\begin{table}[]
\resizebox{1.\linewidth}{!}{
\begin{tabular}{c|ccc|cc|c|cccc}
\hline
\multirow{2}{*}{Task}              & \multicolumn{3}{c|}{{\ul COCO}}                                     & {\ul g-Ref}          & {\ul Entity}          & {\ul VOC}             & \multicolumn{2}{c}{{\ul Karpathy}}          & \multicolumn{2}{c}{{\ul Entity}}            \\
                                   & PQ                   & mAP                  & mIoU                  & cIoU                 & cIoU                  & Point                 & IR@1                 & TR@1                 & IR@1                 & TR@1                 \\ \hline
All                        &   48.5       &    39.0      &    \textbf{61.4}       &    \textbf{61.3}         &  73.0            &     82.6      &      \textbf{40.4}            &      \textbf{54.0}           &          \textbf{50.8}       &     \textbf{51.9}           \\
- Retrieval                        &      48.5                &    39.0                  &            61.1                             &       60.6                &         \textbf{73.2}             &      \textbf{82.8}        & - & -      &          44.3            &     44.8                 \\
- Grounding                        &       48.6               &       39.1               &         61.3              &           -           &          40.9             &               82.8        &         -             &            -          &        45.3              &      46.2                \\
- Interactive                       &        48.6              &         38.8             &           61.0            &          -            &        36.5               &              -         &            -          &         -             &       31.4               &         33.4             \\
- Interleave                       &       \textbf{48.9}               &        \textbf{39.3}              &               61.0        &            -          &       -                &            -           &                   -   &            -          &            -          &             -         \\ \hline
\end{tabular}
}
\vspace{-1pt}
\caption{Ablate on each training task.}
\vspace{-15pt}
\label{tab:aba2}
\end{table}

==> tables/ablation3.tex <==
\begin{table}[]
\resizebox{1.\linewidth}{!}{
\begin{tabular}{c|ccc|cc|c|cccc}
\hline
\multirow{2}{*}{Language Level} & \multicolumn{3}{c|}{{\ul COCO}} & {\ul g-Ref} & {\ul Entity} & {\ul VOC} & \multicolumn{2}{c}{{\ul Karpathy}} & \multicolumn{2}{c}{{\ul Entity}} \\
                                & PQ       & mAP      & mIoU      & cIoU        & cIoU         & Point     & IR@1             & TR@1            & IR@1            & TR@1           \\ \hline
{[}-1{]}                        &   48.3       &    39.1      &    61.2       &    61.3         &  73.0            &     82.6      &      38.9            &      52.2           &          50.3       &     50.8           \\
{[}-6{]}                        &     47.8     &    38.8      &     60.4      &     60.3        &      72.9        &     81.3      &       38.1           &       49.9          &    48.1             &     47.5           \\
{[}-12{]}                        &   \textbf{48.5}       &    \textbf{39.0}      &    \textbf{61.4}       &    61.3         &  \textbf{73.0}            &     \textbf{82.6}      &      \textbf{40.4}            &      \textbf{54.0}           &         \textbf{50.8}       &     \textbf{51.9}           \\
{[}-18{]}                       &   48.2       &    39.0      &     61.1      &     62.2        &   72.6           &     82.2      &         40.1         &        52.7         &     50.6           &   50.5             \\
{[}-24{]}                       &   48.5       &  38.8        &   61.5        &     \textbf{61.6}        &    72.9          &    82.6       &    40.2              &   52.2              &      50.5           &    51.3            \\
{[}-30{]}                       &  48.1        &    39.2      &     61.1      &     60.1        &    73.3          &    82.4       &       37.9           &     49.3            &     49.4            &    50.0            \\ \hline
\end{tabular}
}
\caption{Ablate on LLM feature layers.}
\vspace{-15pt}
\label{tab:aba3}
\end{table}

==> tables/compare_bench.tex <==
\begin{table}[h!]
\resizebox{1.\linewidth}{!}{
\begin{tabular}{llllllll}
\hline
           & Task                        & Engine         & Source     & \#data & Box & Mask & GT \\ \hline
LLaVA      & Visual Question Answering   & GPT4           & COCO       & 80K    & -   & -    & -  \\
MMC4       & Interleave Paragraph        & CLIP           & Web        & 571M   & -   & -    & -  \\
ContextDET & Grounded Question Answering & -              & Flicker30k & 30K    & \cmark   & \xmark    & \cmark  \\
GLaMM      & Grounded Caption            & GPT4+Detectors & SAM        & 11M    & \cmark   & \cmark    & \xmark  \\
FIND       & Grounded Caption            & GPT4           & COCO       & 110K   & \cmark   & \cmark    & \cmark  \\ \hline
\end{tabular}
}
\end{table}
